Learning Human-Human Interactions in Images from Weak Textual Supervision

Interactions between humans are diverse and context-dependent, but previous works have treated them as categorical, disregarding the heavy tail of possible interactions. We propose a new paradigm of learning human-human interactions as free text from a single still image, allowing for flexibility in modeling the unlimited space of situations and relationships between people. To overcome the absence of data labelled specifically for this task, we use knowledge distillation applied to synthetic caption data produced by a large language model without explicit supervision. We show that the pseudo-labels produced by this procedure can be used to train a captioning model to effectively understand human-human interactions in images, as measured by a variety of metrics that measure textual and semantic faithfulness and factual groundedness of our predictions. We further show that our approach outperforms SOTA image captioning and situation recognition models on this task. We will release our code and pseudo-labels along with Waldo and Wenda, a manually-curated test set for still image human-human interaction understanding.

==> figures/labels/labels.tex <==
\begin{figure}
    \centering
        \includegraphics[width=0.995\columnwidth]{figures/labels/labels.png}
    \caption{\textbf{Synthetic caption data generation.} We generate synthetic interaction-caption pairs via in-context learning. In the above figure, captions are shown in red boxes and interaction texts in blue. GPT-Neo is prompted with interaction-caption pairs from Who's Waldo (top left), extracted using syntactic parsing, followed by a new interaction based on data from the CC-News dataset (bottom left). The model proceeds to generate a synthetic caption corresponding to the CC-News interaction, and these synthetic caption-interaction pairs are later used to train an abstractive summarization model.}
    \label{fig:synthetic}
\end{figure}

==> tables/supp_imsitu_results_8beams.tex <==
\begin{table*}[t]
  \centering
  \setlength{\tabcolsep}{3.5pt}
  \def\arraystretch{0.95}
  \begin{tabularx}{1.0\textwidth}{llccccccccccccccccc}
     & &
    {\small \rotatebox[origin=l]{90}{\textbf{Average sim.}}} &
    &
    {\small\rotatebox[origin=l]{90}{socializing}} & {\small\rotatebox[origin=l]{90}{distributing} }& {\small\rotatebox[origin=l]{90}{teaching}} & {\small\rotatebox[origin=l]{90}{communicating}} & {\small\rotatebox[origin=l]{90}{interviewing}} & {\small\rotatebox[origin=l]{90}{lecturing}} &
    {\small\rotatebox[origin=l]{90}{training}} &
    {\small\rotatebox[origin=l]{90}{providing}} &
    {\small\rotatebox[origin=l]{90}{instructing}} &
    {\small\rotatebox[origin=l]{90}{giving}} &
    {\small\rotatebox[origin=l]{90}{pushing}} &
    {\small\rotatebox[origin=l]{90}{helping}} &
    {\small\rotatebox[origin=l]{90}{asking}} &
    {\small\rotatebox[origin=l]{90}{coaching}} &
    {\small\rotatebox[origin=l]{90}{talking}} \\
    \midrule
    \textbf{Results@5} \\
    ENv2 & COCO & 0.26 &  & 0.21 & 0.10 & 0.26 & 0.23 & 0.30 & 0.21 & 0.27 & 0.31 & 0.13 & 0.49 & 0.45 & 0.35 & 0.49 & 0.33 & 0.31 \\% & 0.59 & 0.16 & 0.33 & 0.24 \\
    CLIPCap & COCO  & 0.25 &  & 0.19 & 0.09 & 0.29 & 0.26 & 0.31 & 0.20 & 0.27 & 0.26 & 0.12 & 0.47 & 0.41 & 0.29 & 0.48 & 0.32 & 0.66 \\% & 0.30 & 0.17 & 0.38 & 0.22 \\
    CLIPCap & CC  & 0.35 &  & 0.21 & 0.30 & 0.48 & 0.33 & 0.28 & 0.31 & 0.37 & 0.43 & 0.21 & 0.56 & 0.42 & 0.48 & 0.47 & 0.31 & 0.64 \\% & 0.55 & 0.32 & 0.58 & 0.35 \\
    CLIPCap & CC+WW & 0.18  &  & 0.05 & 0.15 & 0.22 & 0.14 & \textbf{0.60} & 0.16 & 0.17 & 0.22 & 0.11 & 0.46 & 0.15 & 0.21 & 0.22 & 0.15 & 0.24 \\% & 0.13 & 0.11 & 0.17 & 0.26\\
    EncDec &pHHI & \underline{0.40} &  & \textbf{0.30} & \textbf{0.35} & \underline{0.49} & \underline{0.41} & 0.39 & \underline{0.33} & \underline{0.51} & \underline{0.51} & \underline{0.23} & \underline{0.79} & \underline{0.47} & \underline{0.49} & \underline{0.57} & \textbf{0.92} & \underline{0.86} \\% & 0.42 & 0.35 & 0.47 & 0.58 \\
    CLIPCap & CC+pHHI & \textbf{0.44} &  & \underline{0.29} & \textbf{0.35} & \textbf{0.85} & \textbf{0.44} & \underline{0.41} & \textbf{0.40} & \textbf{0.56} & \textbf{0.56} & \textbf{0.27} & \textbf{0.88} & \textbf{0.48} & \textbf{0.56} & \textbf{0.58} & \underline{0.86} & \textbf{0.92} \\% & 0.40 & 0.42 & 0.45 & 0.63 \\
    \midrule
    \textbf{Results@8} \\
    ENv2 & COCO & 0.28 &  & 0.22 & 0.12 & 0.27 & 0.24 & 0.30 & 0.21 & 0.28 & 0.32 & 0.13 & 0.51 & 0.47 & 0.37 & 0.50 & 0.35 & 0.34 \\% & 0.61 & 0.17 & 0.38 & 0.25 \\
    CLIPCap & COCO  & 0.26 &  & 0.20 & 0.10 & 0.31 & 0.27 & 0.31 & 0.21 & 0.28 & 0.26 & 0.12 & 0.48 & 0.43 & 0.31 & 0.49 & 0.32 & 0.67 \\% & 0.31 & 0.18 & 0.39 & 0.23 \\
    CLIPCap & CC  & 0.37 &  & 0.23 & 0.31 & 0.51 & 0.34 & 0.31 & 0.32 & 0.40 & 0.45 & 0.22 & 0.59 & 0.45 & 0.51 & 0.49 & 0.32 & 0.70 \\% & 0.60 & 0.33 & 0.61 & 0.3 \\
    CLIPCap & CC+WW & 0.21 &  & 0.06 & 0.16 & 0.25 & 0.16 & \textbf{0.62} & 0.16 & 0.20 & 0.24 & 0.12 & 0.51 & 0.20 & 0.23 & 0.26 & 0.18 & 0.32 \\% & 0.16 & 0.13 & 0.20 & 0.28 \\
    EncDec & pHHI & \underline{0.44} &  & \textbf{0.33} & \textbf{0.38} & \underline{0.55} & \underline{0.44} & \underline{0.42} & \underline{0.34} & \underline{0.54} & \underline{0.56} & \underline{0.25} & \underline{0.85} & \underline{0.49} & \underline{0.56} & \underline{0.59} & \textbf{0.94} & \underline{0.91} \\% & 0.44 & 0.38 & 0.49 & 0.65 \\
    CLIPCap & CC+pHHI & \textbf{0.47} &  & \textbf{0.33} & \underline{0.37} & \textbf{0.90} & \textbf{0.46} & 0.41 & \textbf{0.43} & \textbf{0.60} & \textbf{0.59} & \textbf{0.29} & \textbf{0.92} & \textbf{0.50} & \textbf{0.59} & \textbf{0.61} & \underline{0.91} & \textbf{0.96} \\% & 0.43 & 0.45 & 0.48 & 0.74 \\
    \bottomrule
  \end{tabularx}
  \vspace{0pt}
  \caption{Results on \textbf{\imsituhhi} for top 5 and 8 beams, as described in Section \ref{sec:imsitu_8beams}.}
\label{tab:imsitu_results_8beams}
\end{table*}

==> tables/supp_wenda_results.tex <==
\begin{table*}[t]
  \centering
  \setlength{\tabcolsep}{5.5pt}
  \def\arraystretch{0.95}
  \begin{tabularx}{0.96\textwidth}{llccccccccccccc}
    \toprule
    & &
    \multicolumn{4}{c}{\textbf{WW}} &
    \multicolumn{4}{c}{\textbf{CC}} &
    \multicolumn{4}{c}{\textbf{COCO}}
    \\
    \cmidrule(lr){3-6}
    \cmidrule(lr){7-10}
    \cmidrule(lr){11-14}
    Method & Training Data & BL$\,\uparrow$ & $p_e \uparrow$ & $p_c \downarrow$ & sim$\,\uparrow$ & BL$\,\uparrow$ & $p_e \uparrow$ & $p_c \downarrow$ & sim$\,\uparrow$ & BL$\,\uparrow$ & $p_e \uparrow$ & $p_c \downarrow$ & sim$\,\uparrow$  \\
    \midrule
\textbf{Results@8} \\
Env2 & COCO & 0.29 & 0.34 & 0.15 & 0.42 & 0.31 & 0.35 & 0.25 & 0.48 & 0.36 & 0.59 & 0.10 & 0.53 \\
Env2 & COCO & 0.32 & 0.53 & 0.18 & 0.43 & 0.30 & 0.41 & 0.25 & 0.47 & 0.35 & 0.55 & 0.21 & 0.50 \\
CLIPCap & CC & 0.38 & 0.47 & 0.17 & 0.48 & 0.32 & 0.35 & 0.19 & 0.53 & 0.34 & 0.26 & 0.11 & 0.45 \\
CLIPCap & CC+WW & 0.34 & 0.22 & 0.48 & 0.35 & 0.36 & 0.42 & 0.10 & 0.33 & 0.35 & 0.34 & 0.06 & 0.25 \\
EncDec & pHHI & \textbf{0.60} & \underline{0.69} & \textbf{0.06} & \textbf{0.69} & \underline{0.55} & \underline{0.72} & \underline{0.05} & \underline{0.64} & \underline{0.50} & \underline{0.66} & \underline{0.04} & \underline{0.61} \\
CLIPCap & CC+pHHI & \textbf{0.60} & \textbf{0.70} & \underline{0.07} & \underline{0.68} & \textbf{0.63} & \textbf{0.81} & \textbf{0.03} &  \textbf{0.72} & \textbf{0.55} & \textbf{0.78} & \textbf{0.03} & \textbf{0.67} \\
    \bottomrule
  \end{tabularx}
  \vspace{5pt}
  \caption{Top-8 results on \textbf{\datasetname{}} split by data source -- Who's Waldo (WW), Conceptual Captions (CC), and COCO Captions -- as described in Section \ref{sec:supp_wenda_source}.}
\label{tab:supp_wenda_results}
\end{table*}

